Finite-size evaporating droplets in weakly compressible homogeneous shear turbulence

We perform interface-resolved simulations of finite-size evaporating droplets in weakly-compressible homogeneous shear turbulence (HST). The study is conducted by varying three dimensionless physical parameters: the initial gas temperature over the critical temperature $T_{g,0}/T_c$, the initial droplet diameter over the Kolmogorov scale $d_0/\eta$ and the surface tension, i.e. the shear-based Weber number, $We_{\mathcal{S}}$. For the smallest $We_{\mathcal{S}}$, we first discuss the impact on the evaporation rate of the three thermodynamic models employed to evaluate the gas thermophysical properties: a constant property model and two variable-properties approaches where either the gas density or all the gas properties are allowed to vary. Taking this last approach as reference, the model assuming constant gas properties and evaluated with the "1/3" rule, is shown to predict the evaporation rate better than the model where the only variable property is the gas density. Moreover, we observe that the well-known Fr\"ossling/Ranz-Marshall correlation underpredicts the Sherwood number at low temperatures, $T_{g,0}/T_c=0.75$. Next, we show that the ratio between the actual evaporation rate in turbulence and the one computed in stagnant condition is always much higher than one for weakly deformable droplets: it decreases with $T_{g,0}/T_c$ without approaching unity at the highest $T_{g,0}/T_c$ considered. This suggests an evaporation enhancement due to turbulence also in conditions typical of combustion applications. Finally, we examine the overall evaporation rate and the local interfacial mass-flux at higher $We_{\mathcal{S}}$, showing a positive correlation between evaporation rate and interfacial curvature, especially at the lowest $T_{g,0}/T_c$.

==> log <==
pdflatex -pdf -f jfm.tex && bibtex jfm && pdflatex -pdf -f jfm.tex && pdflatex -pdf -f jfm.tex
pdflatex: unrecognized option '-pdf'
pdflatex: option '-f' is ambiguous; possibilities: '-fmt' '-file-line-error-style' '-file-line-error'
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./jfm.tex
LaTeX2e <2019-10-01> patch level 3
(./jfm.cls
Document Class: jfm 2007/03/13 v1.28 Journal of Fluid Mechanics document class
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/etoolbox/etoolbox.sty)

Found the 'amsbsy' package on the system, using it.

(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsbsy.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsgen.sty))

Found AMS Euler Roman fonts on the system, but you dont seem to have the
'upmath' package installed. JFM.cls can take advantage of these fonts,
if you use 'upmath' package.



Found AMS Symbol fonts on the system, using the 'amssymb' package.

(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/amsfonts.sty)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/lineno/lineno.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2019/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hycolor/hycolor.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/hycolor/xcolor-patch.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/oberdiek/hopatch.sty)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2019/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2019/texmf-dist/tex/generic/atbegshi/atbegshi.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2019/texmf-dist/tex/latex/atveryend/atveryend.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2019/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2019/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amstext.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/textcomp.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1enc.def
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1enc.dfu)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/nomencl/nomencl.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2019/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/tocbasic.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/scrbase.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/scrlfile.sty))))
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2019/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/dvipsnam.def))
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/tabularx.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/array.sty

LaTeX Warning: Command \@xhline  has changed.
               Check if current package is valid.

)) (/usr/local/texlive/2019/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/adjustbox.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/adjcalc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/trimclip.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/collectbox/collectbox.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/tc-pdftex.def))
(/usr/local/texlive/2019/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/varwidth/varwidth.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/realboxes/realboxes.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/appendix/appendix.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/cancel/cancel.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/epstopdf-pkg/epstopdf.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/grfext/grfext.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg)))
No file jfm.aux.
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/local/texlive/2019/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
)

Package hyperref Warning: Height of page (\paperheight) is invalid (0.0pt),
(hyperref)                using 11in.

(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/umsb.fd)

Package natbib Warning: Citation `dauxois2021confronting' on page 1 undefined o
n input line 109.


Package natbib Warning: Citation `birouk2006current' on page 1 undefined on inp
ut line 109.


Package natbib Warning: Citation `mittal2020flow' on page 1 undefined on input 
line 109.


Package natbib Warning: Citation `balachandar2020host' on page 1 undefined on i
nput line 109.


Package natbib Warning: Citation `bourouiba2021fluid' on page 1 undefined on in
put line 109.


Package natbib Warning: Citation `rosti2020fluid' on page 1 undefined on input 
line 109.


Package natbib Warning: Citation `ng2021growth' on page 1 undefined on input li
ne 109.


Package natbib Warning: Citation `chong2021extended' on page 1 undefined on inp
ut line 109.


Package natbib Warning: Citation `bourouiba2020turbulent' on page 1 undefined o
n input line 109.


Package natbib Warning: Citation `rosti2021turbulence' on page 1 undefined on i
nput line 109.


Package natbib Warning: Citation `wong1992internal' on page 1 undefined on inpu
t line 113.


Package natbib Warning: Citation `mandal2012internal' on page 1 undefined on in
put line 113.


Package natbib Warning: Citation `de2016dense' on page 1 undefined on input lin
e 113.


Package natbib Warning: Citation `villermaux2017fine' on page 1 undefined on in
put line 113.


Package natbib Warning: Citation `sahu2018interaction' on page 1 undefined on i
nput line 113.


Package natbib Warning: Citation `marti2017evaporation' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `verwey2018fuel' on page 1 undefined on input 
line 113.


Package natbib Warning: Citation `verwey2020experimental' on page 1 undefined o
n input line 113.


Package natbib Warning: Citation `kuerten2016point' on page 1 undefined on inpu
t line 113.


Package natbib Warning: Citation `maxey2017simulation' on page 1 undefined on i
nput line 113.


Package natbib Warning: Citation `mashayek1998direct' on page 1 undefined on in
put line 113.


Package natbib Warning: Citation `weiss2018evaporating' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `mashayek1998droplet' on page 1 undefined on i
nput line 113.


Package natbib Warning: Citation `weiss2020evaporating' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `russo2014water' on page 1 undefined on input 
line 113.


Package natbib Warning: Citation `bukhvostova2014comparison' on page 1 undefine
d on input line 113.


Package natbib Warning: Citation `reveillon2007effects' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `wang2021direct' on page 1 undefined on input 
line 113.


Package natbib Warning: Citation `elghobashi2019direct' on page 1 undefined on 
input line 115.


Package natbib Warning: Citation `lupo2020direct' on page 1 undefined on input 
line 115.


Package natbib Warning: Citation `chong2021extended' on page 1 undefined on inp
ut line 115.


Package natbib Warning: Citation `birouk2006current' on page 1 undefined on inp
ut line 115.


Package natbib Warning: Citation `albernaz2017droplet' on page 1 undefined on i
nput line 119.


Package natbib Warning: Citation `dodd2021analysis' on page 1 undefined on inpu
t line 121.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 1 undefined on
 input line 122.


Package natbib Warning: Citation `pumir1996turbulence' on page 1 undefined on i
nput line 122.


Package natbib Warning: Citation `sekimoto2016direct' on page 1 undefined on in
put line 122.


Package natbib Warning: Citation `rosti2019droplets' on page 1 undefined on inp
ut line 122.


Package natbib Warning: Citation `tanaka2017effect' on page 1 undefined on inpu
t line 122.


Package natbib Warning: Citation `yousefi2020modulation' on page 1 undefined on
 input line 122.


Package natbib Warning: Citation `verwey2020experimental' on page 1 undefined o
n input line 127.


Package natbib Warning: Citation `lupo2019immersed' on page 1 undefined on inpu
t line 127.


Package natbib Warning: Citation `lupo2020direct' on page 1 undefined on input 
line 127.


Underfull \vbox (badness 1137) has occurred while \output is active
Underfull \hbox (badness 10000) has occurred while \output is active

[1{/usr/local/texlive/2019/texmf-var/fonts/map/pdftex/updmap/pdftex.map}
Non-PDF special ignored!
<special> papersize=174mm,247mm
]
Underfull \vbox (badness 10000) has occurred while \output is active [2]

Package natbib Warning: Citation `scapin2020volume' on page 3 undefined on inpu
t line 139.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 3 undefined on
 input line 140.


Package natbib Warning: Citation `maxey1982distortion' on page 3 undefined on i
nput line 140.


Package natbib Warning: Citation `wang2019vaporization' on page 3 undefined on 
input line 140.


Package natbib Warning: Citation `ni2021numerical' on page 3 undefined on input
 line 140.


LaTeX Warning: Reference `sec:gov_eqn' on page 3 undefined on input line 144.


LaTeX Warning: Reference `sec:num' on page 3 undefined on input line 144.


LaTeX Warning: Reference `sec:results' on page 3 undefined on input line 144.


LaTeX Warning: Reference `sec:concl' on page 3 undefined on input line 144.


Underfull \vbox (badness 10000) has occurred while \output is active [3]

Package natbib Warning: Citation `majda1985derivation' on page 4 undefined on i
nput line 159.


LaTeX Warning: Reference `eqn:mom1' on page 4 undefined on input line 174.


Package natbib Warning: Citation `reid1987properties' on page 4 undefined on in
put line 174.


LaTeX Warning: Reference `sec:eqn_state' on page 4 undefined on input line 174.



LaTeX Warning: Reference `eqn:mom1' on page 4 undefined on input line 175.


LaTeX Warning: Reference `eqn:vap1' on page 4 undefined on input line 175.


LaTeX Warning: Reference `eqn:int_mfx' on page 4 undefined on input line 175.


LaTeX Warning: Reference `eqn:tmp1' on page 4 undefined on input line 175.


LaTeX Warning: Reference `eqn:tmp1' on page 4 undefined on input line 175.

[4]

LaTeX Warning: Reference `eqn:veldiv1' on page 5 undefined on input line 184.


LaTeX Warning: Reference `eqn:pth1' on page 5 undefined on input line 184.

pdfTeX warning (ext4): destination with the same identifier (name{equation.2.1}
) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                 

LaTeX Warning: Reference `eqn:veldiv1' on page 5 undefined on input line 193.


LaTeX Warning: Reference `eqn:pth1' on page 5 undefined on input line 193.


LaTeX Warning: Reference `f_aux' on page 5 undefined on input line 193.


LaTeX Warning: Reference `sec:vel_div' on page 5 undefined on input line 193.


LaTeX Warning: Reference `eqn:mom1' on page 5 undefined on input line 196.


LaTeX Warning: Reference `eqn:vap1' on page 5 undefined on input line 196.


LaTeX Warning: Reference `eqn:int_mfx' on page 5 undefined on input line 196.


LaTeX Warning: Reference `eqn:tmp1' on page 5 undefined on input line 196.


LaTeX Warning: Reference `eqn:veldiv1' on page 5 undefined on input line 196.


LaTeX Warning: Reference `eqn:pth1' on page 5 undefined on input line 196.


LaTeX Warning: Reference `fig:box_shear' on page 5 undefined on input line 196.


[5]

LaTeX Warning: Reference `eqn:decomp' on page 6 undefined on input line 234.


LaTeX Warning: Reference `eqn:mom1' on page 6 undefined on input line 234.


LaTeX Warning: Reference `eqn:decomp' on page 6 undefined on input line 240.


LaTeX Warning: Reference `eqn:tmp3' on page 6 undefined on input line 248.


LaTeX Warning: Reference `eqn:vap3' on page 6 undefined on input line 248.


Package natbib Warning: Citation `leonard1979stable' on page 6 undefined on inp
ut line 254.


Package natbib Warning: Citation `scapin2020volume' on page 6 undefined on inpu
t line 254.


Package natbib Warning: Citation `dalla2020interface' on page 6 undefined on in
put line 254.


Package natbib Warning: Citation `costa2018fft' on page 6 undefined on input li
ne 255.


LaTeX Warning: Reference `sec:val_lm' on page 6 undefined on input line 255.

[6 <./figures/fig1-eps-converted-to.pdf>]

Package natbib Warning: Citation `ii2012interface' on page 7 undefined on input
 line 258.


Package natbib Warning: Citation `rosti2019numerical' on page 7 undefined on in
put line 258.


LaTeX Warning: Reference `eqn:phase_ind' on page 7 undefined on input line 258.



Package natbib Warning: Citation `scapin2020volume' on page 7 undefined on inpu
t line 263.


LaTeX Warning: Reference `eqn:decomp' on page 7 undefined on input line 263.


LaTeX Warning: Reference `eqn:phi' on page 7 undefined on input line 264.


LaTeX Warning: Reference `eqn:decomp' on page 7 undefined on input line 264.


LaTeX Warning: Reference `eqn:phi' on page 7 undefined on input line 264.


LaTeX Warning: Reference `eqn:phi1' on page 7 undefined on input line 269.


LaTeX Warning: Reference `eqn:phi1' on page 7 undefined on input line 270.


Package natbib Warning: Citation `ii2012interface' on page 7 undefined on input
 line 270.


LaTeX Warning: Reference `eqn:phi2' on page 7 undefined on input line 275.


LaTeX Warning: Reference `eqn:phi2' on page 7 undefined on input line 275.

[7]

Package natbib Warning: Citation `scapin2020volume' on page 8 undefined on inpu
t line 282.


LaTeX Warning: Reference `eqn:vap3' on page 8 undefined on input line 285.


LaTeX Warning: Reference `eqn:sp_wg_1' on page 8 undefined on input line 286.


LaTeX Warning: Reference `eqn:sp_wg_2' on page 8 undefined on input line 286.


LaTeX Warning: Reference `sec:eqn_state' on page 8 undefined on input line 286.



LaTeX Warning: Reference `eqn:vap3' on page 8 undefined on input line 286.


LaTeX Warning: Reference `eqn:vap3_disc' on page 8 undefined on input line 291.



Package natbib Warning: Citation `scapin2020volume' on page 8 undefined on inpu
t line 291.


Package natbib Warning: Citation `scapin2020volume' on page 8 undefined on inpu
t line 295.


LaTeX Warning: Reference `eqn:alphag' on page 8 undefined on input line 305.


LaTeX Warning: Reference `eqn:alphag' on page 8 undefined on input line 305.


LaTeX Warning: Reference `sec:eqn_state' on page 8 undefined on input line 308.


[8]

LaTeX Warning: Reference `eqn:yvap_rem' on page 9 undefined on input line 314.


Package natbib Warning: Citation `gerz1989direct' on page 9 undefined on input 
line 314.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 9 undefined on
 input line 314.


LaTeX Warning: Reference `eqn:yv' on page 9 undefined on input line 319.


Package natbib Warning: Citation `tanaka2017effect' on page 9 undefined on inpu
t line 319.


LaTeX Warning: Reference `sec:time_step' on page 9 undefined on input line 319.



LaTeX Warning: Reference `eqn:int_mfx' on page 9 undefined on input line 322.


LaTeX Warning: Reference `sec:vap_mass' on page 9 undefined on input line 322.


LaTeX Warning: Reference `sec:eqn_state' on page 9 undefined on input line 326.



LaTeX Warning: Reference `eqn:veldiv1' on page 9 undefined on input line 326.


LaTeX Warning: Reference `eqn:tmp1' on page 9 undefined on input line 330.


Package natbib Warning: Citation `scapin2020volume' on page 9 undefined on inpu
t line 330.


Package natbib Warning: Citation `gerz1989direct' on page 9 undefined on input 
line 330.


LaTeX Warning: Reference `sec:imp_ab2' on page 9 undefined on input line 338.

[9]

LaTeX Warning: Reference `eqn:tmp1' on page 10 undefined on input line 344.


LaTeX Warning: Reference `eqn:tmp_disc' on page 10 undefined on input line 352.



LaTeX Warning: Reference `eqn:remap_tmp' on page 10 undefined on input line 352
.


LaTeX Warning: Reference `eqn:veldiv1' on page 10 undefined on input line 355.


Package natbib Warning: Citation `dalla2020interface' on page 10 undefined on i
nput line 355.


LaTeX Warning: Reference `eqn:veldiv1' on page 10 undefined on input line 356.


LaTeX Warning: Reference `gas_density' on page 10 undefined on input line 356.


LaTeX Warning: Reference `sec:eqn_state' on page 10 undefined on input line 356
.


Package natbib Warning: Citation `demou2019low' on page 10 undefined on input l
ine 356.


Package natbib Warning: Citation `dalla2020interface' on page 10 undefined on i
nput line 356.


LaTeX Warning: Reference `eqn:cal_mg1' on page 10 undefined on input line 365.


LaTeX Warning: Reference `eqn:cal_mg1' on page 10 undefined on input line 365.


LaTeX Warning: Reference `eqn:cal_mg2' on page 10 undefined on input line 370.

[10]

LaTeX Warning: Reference `eqn:mom1' on page 11 undefined on input line 373.


LaTeX Warning: Reference `eqn:u_predic' on page 11 undefined on input line 383.



LaTeX Warning: Reference `sec:imp_ab2' on page 11 undefined on input line 383.


Package natbib Warning: Citation `rosti2019droplets' on page 11 undefined on in
put line 383.


LaTeX Warning: Reference `eqn:lap_p' on page 11 undefined on input line 384.


Package natbib Warning: Citation `dodd2014fast' on page 11 undefined on input l
ine 384.


LaTeX Warning: Reference `eqn:lap_p' on page 11 undefined on input line 385.


LaTeX Warning: Reference `eqn:corr' on page 11 undefined on input line 385.


Package natbib Warning: Citation `motheau2016high' on page 11 undefined on inpu
t line 385.


Package natbib Warning: Citation `dalla2020interface' on page 11 undefined on i
nput line 385.


LaTeX Warning: Reference `eqn:lap_p' on page 11 undefined on input line 385.


LaTeX Warning: Reference `eqn:lap_p' on page 11 undefined on input line 385.


Package natbib Warning: Citation `tanaka2017effect' on page 11 undefined on inp
ut line 385.


Package natbib Warning: Citation `rosti2019droplets' on page 11 undefined on in
put line 385.


Package natbib Warning: Citation `scapin2020volume' on page 11 undefined on inp
ut line 398.


Package natbib Warning: Citation `dalla2020interface' on page 11 undefined on i
nput line 398.

[11]
Overfull \hbox (9.16872pt too wide) in paragraph at lines 425--479
[]$[]$  $[]$ 

LaTeX Warning: Reference `eqn:dav' on page 12 undefined on input line 479.


LaTeX Warning: Reference `eqn:dav' on page 12 undefined on input line 479.


Package natbib Warning: Citation `hubbard1975droplet' on page 12 undefined on i
nput line 482.


LaTeX Warning: Reference `tab:param' on page 12 undefined on input line 482.


LaTeX Warning: Reference `tab:param' on page 12 undefined on input line 482.

[12]

Package natbib Warning: Citation `sekimoto2016direct' on page 13 undefined on i
nput line 484.


Package natbib Warning: Citation `scapin2020volume' on page 13 undefined on inp
ut line 484.


Package natbib Warning: Citation `abramzon1989droplet' on page 13 undefined on 
input line 491.


Package natbib Warning: Citation `lupo2019immersed' on page 13 undefined on inp
ut line 491.


Package natbib Warning: Citation `lupo2020direct' on page 13 undefined on input
 line 491.


Package natbib Warning: Citation `hubbard1975droplet' on page 13 undefined on i
nput line 491.


Package natbib Warning: Citation `langmuir1918evaporation' on page 13 undefined
 on input line 491.


LaTeX Warning: Reference `eqn:veldiv1' on page 13 undefined on input line 491.


LaTeX Warning: Reference `eqn:pth1' on page 13 undefined on input line 491.


Package natbib Warning: Citation `piedra2015numerical' on page 13 undefined on 
input line 491.


LaTeX Warning: Reference `fig:d2' on page 13 undefined on input line 494.


LaTeX Warning: Reference `fig:rho_g' on page 13 undefined on input line 494.


LaTeX Warning: Reference `fig:tmpg' on page 13 undefined on input line 494.


LaTeX Warning: Reference `fig:tmpg' on page 13 undefined on input line 494.


LaTeX Warning: Reference `fig:d2' on page 13 undefined on input line 535.


LaTeX Warning: Reference `fig:area' on page 13 undefined on input line 535.

[13] [14 <./figures/fig2-eps-converted-to.pdf> <./figures/fig3-eps-converted-to
.pdf>]

Package natbib Warning: Citation `birouk2006current' on page 15 undefined on in
put line 549.


Package natbib Warning: Citation `abramzon1989droplet' on page 15 undefined on 
input line 549.


LaTeX Warning: Reference `eqn:klam' on page 15 undefined on input line 555.


Package natbib Warning: Citation `ranz1952evaporation' on page 15 undefined on 
input line 555.


Package natbib Warning: Citation `birouk2006current' on page 15 undefined on in
put line 555.

[15 <./figures/fig4-eps-converted-to.pdf> <./figures/fig5-eps-converted-to.pdf>
 <./figures/fig6-eps-converted-to.pdf>]

Package natbib Warning: Citation `ranz1952evaporation' on page 16 undefined on 
input line 563.


Package natbib Warning: Citation `wang2021direct' on page 16 undefined on input
 line 563.


Package natbib Warning: Citation `ng2021growth' on page 16 undefined on input l
ine 563.


Package natbib Warning: Citation `ng2021growth' on page 16 undefined on input l
ine 563.


LaTeX Warning: Reference `eqn:klam' on page 16 undefined on input line 564.


Package natbib Warning: Citation `gokalp1992mass' on page 16 undefined on input
 line 564.


Package natbib Warning: Citation `abramzon1989droplet' on page 16 undefined on 
input line 574.


Package natbib Warning: Citation `birouk2006current' on page 16 undefined on in
put line 574.


Package natbib Warning: Citation `abramzon1989droplet' on page 16 undefined on 
input line 580.


LaTeX Warning: Reference `eqn:klam' on page 16 undefined on input line 580.


LaTeX Warning: Reference `eqn:sh_pp' on page 16 undefined on input line 580.


LaTeX Warning: Reference `fig:d2' on page 16 undefined on input line 581.


LaTeX Warning: Reference `eqn:klam' on page 16 undefined on input line 582.


Package natbib Warning: Citation `lupo2020uncertainty' on page 16 undefined on 
input line 582.

[16 <./figures/fig7-eps-converted-to.pdf> <./figures/fig8-eps-converted-to.pdf>
]

LaTeX Warning: Reference `fig:sh' on page 17 undefined on input line 585.


LaTeX Warning: Reference `eqn:sh1' on page 17 undefined on input line 590.

[17 <./figures/fig9-eps-converted-to.pdf> <./figures/fig10-eps-converted-to.pdf
>]

LaTeX Warning: Reference `fig:sh' on page 18 undefined on input line 609.


LaTeX Warning: Reference `tab:param' on page 18 undefined on input line 609.


Package natbib Warning: Citation `mees2020statistical' on page 18 undefined on 
input line 610.


Package natbib Warning: Citation `lupo2020direct' on page 18 undefined on input
 line 610.


LaTeX Warning: Reference `fig:d2_diff_re' on page 18 undefined on input line 61
6.


Package natbib Warning: Citation `verwey2018fuel' on page 18 undefined on input
 line 616.


Package natbib Warning: Citation `verwey2020experimental' on page 18 undefined 
on input line 616.


Package natbib Warning: Citation `marti2017evaporation' on page 18 undefined on
 input line 616.


LaTeX Warning: Reference `fig:d2_diff_re' on page 18 undefined on input line 61
6.


Package natbib Warning: Citation `birouk2006current' on page 18 undefined on in
put line 616.


LaTeX Warning: Reference `fig:ts_nu_ht' on page 18 undefined on input line 633.



LaTeX Warning: Reference `fig:ts_nu_ht' on page 18 undefined on input line 634.



LaTeX Warning: Reference `fig:ts_nu_ht' on page 18 undefined on input line 635.



LaTeX Warning: Reference `fig:ts_nu_ht' on page 18 undefined on input line 636.


[18]

Package natbib Warning: Citation `ni2021numerical' on page 19 undefined on inpu
t line 707.


LaTeX Warning: Reference `eqn:fluxes' on page 19 undefined on input line 709.

[19 <./figures/fig11-eps-converted-to.pdf> <./figures/fig12-eps-converted-to.pd
f>]

LaTeX Warning: Reference `fig:hist_tmp_out' on page 20 undefined on input line 
749.


LaTeX Warning: Reference `sec:3model' on page 20 undefined on input line 749.


LaTeX Warning: Reference `fig:hist_tmp_in' on page 20 undefined on input line 7
49.


Package natbib Warning: Citation `wong1992internal' on page 20 undefined on inp
ut line 749.


Package natbib Warning: Citation `pinheiro2019ethanol' on page 20 undefined on 
input line 749.


LaTeX Warning: Reference `fig:hist_sca_out' on page 20 undefined on input line 
749.

[20 <./figures/fig13-eps-converted-to.pdf> <./figures/fig14-eps-converted-to.pd
f> <./figures/fig15-eps-converted-to.pdf>]

LaTeX Warning: Reference `sec:3model' on page 21 undefined on input line 771.


LaTeX Warning: Reference `sec:3model' on page 21 undefined on input line 771.


LaTeX Warning: Reference `fig:d2_diff_we' on page 21 undefined on input line 77
7.


LaTeX Warning: Reference `fig:d2_diff_we' on page 21 undefined on input line 77
7.

[21 <./figures/fig16-eps-converted-to.pdf> <./figures/fig17-eps-converted-to.pd
f> <./figures/fig18-eps-converted-to.pdf> <./figures/fig19-eps-converted-to.pdf
>]

LaTeX Warning: Reference `fig:area_diff_we' on page 22 undefined on input line 
797.


LaTeX Warning: Reference `fig:pi_sigma_n' on page 22 undefined on input line 80
3.


LaTeX Warning: Reference `fig:pi_sigma_n' on page 22 undefined on input line 80
5.


LaTeX Warning: Reference `fig:d2_diff_we' on page 22 undefined on input line 80
5.

[22 <./figures/fig20-eps-converted-to.pdf> <./figures/fig21-eps-converted-to.pd
f>]

Package natbib Warning: Citation `tonini2013exact' on page 23 undefined on inpu
t line 831.


Package natbib Warning: Citation `saenz2017dynamics' on page 23 undefined on in
put line 831.

[23 <./figures/fig22-eps-converted-to.pdf> <./figures/fig23-eps-converted-to.pd
f> <./figures/fig24-eps-converted-to.pdf>]

LaTeX Warning: Reference `eqn:int_mfx' on page 24 undefined on input line 836.


LaTeX Warning: Reference `fig:jpdf_mk_lw_hr' on page 24 undefined on input line
 837.

[24 <./figures/fig25-eps-converted-to.pdf> <./figures/fig26-eps-converted-to.pd
f> <./figures/fig27-eps-converted-to.pdf>]

LaTeX Warning: Reference `fig:jpdf_mk_lw_hr' on page 25 undefined on input line
 869.


LaTeX Warning: Reference `fig:jpdf_mk_lr' on page 25 undefined on input line 87
4.


LaTeX Warning: Reference `fig:jpdf_mk_lw_hr' on page 25 undefined on input line
 875.


LaTeX Warning: Reference `fig:jpdf_mk_hw_hr' on page 25 undefined on input line
 875.

[25 <./figures/fig28-eps-converted-to.pdf> <./figures/fig29-eps-converted-to.pd
f>]

Package natbib Warning: Citation `kasbaoui2017algorithm' on page 26 undefined o
n input line 880.


Package natbib Warning: Citation `ranz1952evaporation' on page 26 undefined on 
input line 890.


Package natbib Warning: Citation `mees2020statistical' on page 26 undefined on 
input line 890.


Package natbib Warning: Citation `tonini2013exact' on page 26 undefined on inpu
t line 900.


Package natbib Warning: Citation `saenz2017dynamics' on page 26 undefined on in
put line 900.

[26 <./figures/fig30-eps-converted-to.pdf>]
Overfull \hbox (16.66757pt too wide) in paragraph at lines 916--922
[]\OT1/cmr/m/n/10 N. Scapin, https://orcid.org/0000-0002-1330-3348; F. Dalla Ba
rba, https://orcid.org/0000-

Underfull \hbox (badness 1960) in paragraph at lines 916--922
\OT1/cmr/m/n/10 0002-4262-0537; Gi-an-domenico Lupo, https://orcid.org/0000-000
2-1095-118X; M.E.
[27]

Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 944.


Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 952.


Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 960.


Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 968.


LaTeX Warning: Reference `sec:vap_mass' on page 28 undefined on input line 975.


[28]

Package natbib Warning: Citation `span1996new' on page 29 undefined on input li
ne 980.


Package natbib Warning: Citation `span1996new' on page 29 undefined on input li
ne 985.


LaTeX Warning: Reference `sec:re_effect' on page 29 undefined on input line 988
.


Package natbib Warning: Citation `reid1987properties' on page 29 undefined on i
nput line 988.


LaTeX Warning: Reference `eqn:mom1' on page 29 undefined on input line 992.


LaTeX Warning: Reference `eqn:vap1' on page 29 undefined on input line 992.


LaTeX Warning: Reference `eqn:int_mfx' on page 29 undefined on input line 992.


LaTeX Warning: Reference `eqn:tmp1' on page 29 undefined on input line 992.


LaTeX Warning: Reference `sec:gov_eqn' on page 29 undefined on input line 992.


Package natbib Warning: Citation `majda1985derivation' on page 29 undefined on 
input line 992.


Package natbib Warning: Citation `dodd2021analysis' on page 29 undefined on inp
ut line 992.

[29]

LaTeX Warning: Reference `total_jump' on page 30 undefined on input line 1014.


LaTeX Warning: Reference `jump_n' on page 30 undefined on input line 1014.


LaTeX Warning: Reference `div_u' on page 30 undefined on input line 1014.


LaTeX Warning: Reference `div_u' on page 30 undefined on input line 1020.


LaTeX Warning: Reference `gas_density' on page 30 undefined on input line 1024.



LaTeX Warning: Reference `div_u1' on page 30 undefined on input line 1031.


LaTeX Warning: Reference `drhogdt' on page 30 undefined on input line 1031.


Package natbib Warning: Citation `dodd2021analysis' on page 30 undefined on inp
ut line 1031.


LaTeX Warning: Reference `divug' on page 30 undefined on input line 1036.


LaTeX Warning: Reference `div_u' on page 30 undefined on input line 1037.


Package natbib Warning: Citation `motheau2016high' on page 30 undefined on inpu
t line 1038.


LaTeX Warning: Reference `divug' on page 30 undefined on input line 1038.


LaTeX Warning: Reference `eqn:vap1' on page 30 undefined on input line 1038.


Package natbib Warning: Citation `reid1987properties' on page 30 undefined on i
nput line 1038.


LaTeX Warning: Reference `divug' on page 30 undefined on input line 1038.

[30]

LaTeX Warning: Reference `eqn:enthalpy' on page 31 undefined on input line 1048
.


Package natbib Warning: Citation `lupo2019immersed' on page 31 undefined on inp
ut line 1056.


LaTeX Warning: Reference `eqn:lupo_dev' on page 31 undefined on input line 1061
.


LaTeX Warning: Reference `eqn:ent_split' on page 31 undefined on input line 106
1.


LaTeX Warning: Reference `eqn:enthalpy' on page 31 undefined on input line 1061
.


LaTeX Warning: Reference `eqn:vap1' on page 31 undefined on input line 1061.


LaTeX Warning: Reference `eqn:tmp' on page 31 undefined on input line 1066.


LaTeX Warning: Reference `eqn:tmp1' on page 31 undefined on input line 1066.


LaTeX Warning: Reference `eqn:tmp' on page 31 undefined on input line 1066.


LaTeX Warning: Reference `eqn:vap_mass' on page 31 undefined on input line 1066
.


LaTeX Warning: Reference `divug' on page 31 undefined on input line 1066.


LaTeX Warning: Reference `div_u' on page 31 undefined on input line 1066.

[31]

LaTeX Warning: Reference `eqn:kinematic' on page 32 undefined on input line 108
4.


Package natbib Warning: Citation `scapin2020volume' on page 32 undefined on inp
ut line 1101.


LaTeX Warning: Reference `eqn:veldiv' on page 32 undefined on input line 1101.


LaTeX Warning: Reference `eqn:dt' on page 32 undefined on input line 1106.


LaTeX Warning: Reference `eqn:pth_ex' on page 32 undefined on input line 1107.


LaTeX Warning: Reference `fig:validation1' on page 32 undefined on input line 1
107.


Package natbib Warning: Citation `ni2021numerical' on page 32 undefined on inpu
t line 1148.


Package natbib Warning: Citation `ni2021numerical' on page 32 undefined on inpu
t line 1148.


LaTeX Warning: Reference `fig:validation23' on page 32 undefined on input line 
1148.

[32]

Package natbib Warning: Citation `verwey2018fuel' on page 33 undefined on input
 line 1148.


Package natbib Warning: Citation `dodd2021analysis' on page 33 undefined on inp
ut line 1148.


Package natbib Warning: Citation `podvigina1994non' on page 33 undefined on inp
ut line 1148.


LaTeX Warning: Reference `fig:validation23' on page 33 undefined on input line 
1148.


Package natbib Warning: Citation `verwey2018fuel' on page 33 undefined on input
 line 1148.


LaTeX Warning: Reference `subsec:hexadecane' on page 33 undefined on input line
 1148.


LaTeX Warning: Reference `subsec:heptane' on page 33 undefined on input line 11
48.


LaTeX Warning: Reference `subsec:hexadecane' on page 33 undefined on input line
 1148.


LaTeX Warning: Reference `subsec:heptane' on page 33 undefined on input line 11
48.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 33 undefined o
n input line 1151.


Package natbib Warning: Citation `gerz1989direct' on page 33 undefined on input
 line 1151.


Package natbib Warning: Citation `maxey1982distortion' on page 33 undefined on 
input line 1151.


Package natbib Warning: Citation `isaza2009asymptotic' on page 33 undefined on 
input line 1151.

[33 <./figures/fig31-eps-converted-to.pdf> <./figures/fig32-eps-converted-to.pd
f>]

Package natbib Warning: Citation `kasbaoui2017algorithm' on page 34 undefined o
n input line 1155.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 34 undefined o
n input line 1161.


LaTeX Warning: Reference `eqn:toy_hst' on page 34 undefined on input line 1161.



Package natbib Warning: Citation `maxey1982distortion' on page 34 undefined on 
input line 1161.


LaTeX Warning: Reference `eqn:toy_hst' on page 34 undefined on input line 1161.



Package natbib Warning: Citation `gerz1989direct' on page 34 undefined on input
 line 1182.


LaTeX Warning: Reference `err' on page 34 undefined on input line 1182.


Underfull \hbox (badness 1642) in paragraph at lines 1180--1183
\OT1/cmr/m/n/10 Following the ap-proach pro-posed by \OT1/cmr/bx/n/10 ?\OT1/cmr
/m/n/10 , we set $[]([]\OML/cmm/m/it/10 ; \OT1/cmr/bx/n/10 k[]\OT1/cmr/m/n/10 )
 = [] [](\OML/cmm/m/it/10 i\OT1/cmr/bx/n/10 k[] \OMS/cmsy/m/n/10 ^^A \OT1/cmr/b
x/n/10 x\OT1/cmr/m/n/10 )$

Underfull \hbox (badness 2653) in paragraph at lines 1180--1183
\OT1/cmr/m/n/10 and $[]([]\OML/cmm/m/it/10 ; \OT1/cmr/bx/n/10 k[]\OT1/cmr/m/n/1
0 ) = [] [](\OML/cmm/m/it/10 i\OT1/cmr/bx/n/10 k[] \OMS/cmsy/m/n/10 ^^A \OT1/cm
r/bx/n/10 x\OT1/cmr/m/n/10 )$. More-over, by us-ing the iden-tity
[34pdfTeX warning (ext4): destination with the same identifier (name{equation.D
.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1186 \end{equation}
                     pdfTeX warning (ext4): destination with the same identifie
r (name{equation.D.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1186 \end{equation}
                      <./figures/fig33-eps-converted-to.pdf> <./figures/fig34-e
ps-converted-to.pdf>]

LaTeX Warning: Reference `err_n1a' on page 35 undefined on input line 1194.


LaTeX Warning: Reference `eqn:first_cond' on page 35 undefined on input line 11
94.


LaTeX Warning: Reference `eqn:sec_cond' on page 35 undefined on input line 1198
.


Package natbib Warning: Citation `gerz1989direct' on page 35 undefined on input
 line 1199.


LaTeX Warning: Reference `err' on page 35 undefined on input line 1199.


LaTeX Warning: Reference `err_rosti' on page 35 undefined on input line 1204.


LaTeX Warning: Reference `err_rosti' on page 35 undefined on input line 1204.


LaTeX Warning: Reference `err' on page 35 undefined on input line 1204.


LaTeX Warning: Reference `err_n1' on page 35 undefined on input line 1209.


LaTeX Warning: Reference `err_n0' on page 35 undefined on input line 1214.


LaTeX Warning: Reference `err_n1_rosti' on page 35 undefined on input line 1214
.


LaTeX Warning: Reference `eqn:sec_cond' on page 35 undefined on input line 1214
.


LaTeX Warning: Reference `eqn:first_cond' on page 35 undefined on input line 12
14.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 35 undefined o
n input line 1230.


LaTeX Warning: Reference `rdt_2d' on page 35 undefined on input line 1230.


Package natbib Warning: Citation `tanaka2017effect' on page 35 undefined on inp
ut line 1231.


Package natbib Warning: Citation `yousefi2020modulation' on page 35 undefined o
n input line 1231.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 35 undefined o
n input line 1231.


LaTeX Warning: Reference `fig:ab2_r' on page 35 undefined on input line 1257.


LaTeX Warning: Reference `fig:cn2' on page 35 undefined on input line 1257.


LaTeX Warning: Reference `fig:ab2_g' on page 35 undefined on input line 1258.

[35] [36 <./figures/fig35-eps-converted-to.pdf> <./figures/fig36-eps-converted-
to.pdf> <./figures/fig37-eps-converted-to.pdf>]

LaTeX Warning: Reference `fig:rdt_sol' on page 37 undefined on input line 1277.



LaTeX Warning: Reference `fig:error' on page 37 undefined on input line 1277.


LaTeX Warning: Reference `fig:ab2_g' on page 37 undefined on input line 1278.

No file jfm.bbl.

Package natbib Warning: There were undefined citations.

[37 <./figures/fig38-eps-converted-to.pdf> <./figures/fig39-eps-converted-to.pd
f>] (./jfm.aux)

Package rerunfilecheck Warning: File `jfm.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.


LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information){/usr/local/texlive/2019/te
xmf-dist/fonts/enc/dvips/cm-super/cm-super-ts1.enc}</usr/local/texlive/2019/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2019/texm
f-dist/fonts/type1/public/amsfonts/cm/cmbx12.pfb></usr/local/texlive/2019/texmf
-dist/fonts/type1/public/amsfonts/cm/cmbx7.pfb></usr/local/texlive/2019/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmbx8.pfb></usr/local/texlive/2019/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2019/texmf-dist
/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2019/texmf-dist/
fonts/type1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2019/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2019/texmf-dist/font
s/type1/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2019/texmf-dist/fonts/
type1/public/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2019/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type
1/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmr6.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/publ
ic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/
amsfonts/cm/cmr9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsf
onts/cm/cmsy5.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfon
ts/cm/cmsy6.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts
/cm/cmsy7.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/c
m/cmsy9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/
cmti10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/c
mti8.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/cmt
i9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/symbols/
msam10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/cm-super/sfrm
1000.pfb>
Output written on jfm.pdf (37 pages, 8895725 bytes).
Transcript written on jfm.log.
This is BibTeX, Version 0.99d (TeX Live 2019)
The top-level auxiliary file: jfm.aux
The style file: jfm.bst
Database file #1: bibfile.bib
Warning--empty journal in reid1987properties
(There was 1 warning)
pdflatex: unrecognized option '-pdf'
pdflatex: option '-f' is ambiguous; possibilities: '-fmt' '-file-line-error-style' '-file-line-error'
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./jfm.tex
LaTeX2e <2019-10-01> patch level 3
(./jfm.cls
Document Class: jfm 2007/03/13 v1.28 Journal of Fluid Mechanics document class
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/etoolbox/etoolbox.sty)

Found the 'amsbsy' package on the system, using it.

(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsbsy.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsgen.sty))

Found AMS Euler Roman fonts on the system, but you dont seem to have the
'upmath' package installed. JFM.cls can take advantage of these fonts,
if you use 'upmath' package.



Found AMS Symbol fonts on the system, using the 'amssymb' package.

(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/amsfonts.sty)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/lineno/lineno.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2019/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hycolor/hycolor.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/hycolor/xcolor-patch.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/oberdiek/hopatch.sty)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2019/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2019/texmf-dist/tex/generic/atbegshi/atbegshi.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2019/texmf-dist/tex/latex/atveryend/atveryend.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2019/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2019/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amstext.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/textcomp.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1enc.def
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1enc.dfu)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/nomencl/nomencl.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2019/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/tocbasic.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/scrbase.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/scrlfile.sty))))
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2019/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/dvipsnam.def))
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/tabularx.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/array.sty

LaTeX Warning: Command \@xhline  has changed.
               Check if current package is valid.

)) (/usr/local/texlive/2019/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/adjustbox.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/adjcalc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/trimclip.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/collectbox/collectbox.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/tc-pdftex.def))
(/usr/local/texlive/2019/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/varwidth/varwidth.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/realboxes/realboxes.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/appendix/appendix.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/cancel/cancel.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/epstopdf-pkg/epstopdf.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/grfext/grfext.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg)))
(./jfm.aux

LaTeX Warning: Label `eqn:veldiv' multiply defined.

) (/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/local/texlive/2019/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
)

Package hyperref Warning: Height of page (\paperheight) is invalid (0.0pt),
(hyperref)                using 11in.

(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./jfm.out) (./jfm.out)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/umsb.fd)

Package natbib Warning: Citation `dauxois2021confronting' on page 1 undefined o
n input line 109.


Package natbib Warning: Citation `birouk2006current' on page 1 undefined on inp
ut line 109.


Package natbib Warning: Citation `mittal2020flow' on page 1 undefined on input 
line 109.


Package natbib Warning: Citation `balachandar2020host' on page 1 undefined on i
nput line 109.


Package natbib Warning: Citation `bourouiba2021fluid' on page 1 undefined on in
put line 109.


Package natbib Warning: Citation `rosti2020fluid' on page 1 undefined on input 
line 109.


Package natbib Warning: Citation `ng2021growth' on page 1 undefined on input li
ne 109.


Package natbib Warning: Citation `chong2021extended' on page 1 undefined on inp
ut line 109.


Package natbib Warning: Citation `bourouiba2020turbulent' on page 1 undefined o
n input line 109.


Package natbib Warning: Citation `rosti2021turbulence' on page 1 undefined on i
nput line 109.


Package natbib Warning: Citation `wong1992internal' on page 1 undefined on inpu
t line 113.


Package natbib Warning: Citation `mandal2012internal' on page 1 undefined on in
put line 113.


Package natbib Warning: Citation `de2016dense' on page 1 undefined on input lin
e 113.


Package natbib Warning: Citation `villermaux2017fine' on page 1 undefined on in
put line 113.


Package natbib Warning: Citation `sahu2018interaction' on page 1 undefined on i
nput line 113.


Package natbib Warning: Citation `marti2017evaporation' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `verwey2018fuel' on page 1 undefined on input 
line 113.


Package natbib Warning: Citation `verwey2020experimental' on page 1 undefined o
n input line 113.


Package natbib Warning: Citation `kuerten2016point' on page 1 undefined on inpu
t line 113.


Package natbib Warning: Citation `maxey2017simulation' on page 1 undefined on i
nput line 113.


Package natbib Warning: Citation `mashayek1998direct' on page 1 undefined on in
put line 113.


Package natbib Warning: Citation `weiss2018evaporating' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `mashayek1998droplet' on page 1 undefined on i
nput line 113.


Package natbib Warning: Citation `weiss2020evaporating' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `russo2014water' on page 1 undefined on input 
line 113.


Package natbib Warning: Citation `bukhvostova2014comparison' on page 1 undefine
d on input line 113.


Package natbib Warning: Citation `reveillon2007effects' on page 1 undefined on 
input line 113.


Package natbib Warning: Citation `wang2021direct' on page 1 undefined on input 
line 113.


Package natbib Warning: Citation `elghobashi2019direct' on page 1 undefined on 
input line 115.


Package natbib Warning: Citation `lupo2020direct' on page 1 undefined on input 
line 115.


Package natbib Warning: Citation `chong2021extended' on page 1 undefined on inp
ut line 115.


Package natbib Warning: Citation `birouk2006current' on page 1 undefined on inp
ut line 115.


Package natbib Warning: Citation `albernaz2017droplet' on page 1 undefined on i
nput line 119.


Package natbib Warning: Citation `dodd2021analysis' on page 1 undefined on inpu
t line 121.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 1 undefined on
 input line 122.


Package natbib Warning: Citation `pumir1996turbulence' on page 1 undefined on i
nput line 122.


Package natbib Warning: Citation `sekimoto2016direct' on page 1 undefined on in
put line 122.


Package natbib Warning: Citation `rosti2019droplets' on page 1 undefined on inp
ut line 122.


Package natbib Warning: Citation `tanaka2017effect' on page 1 undefined on inpu
t line 122.


Package natbib Warning: Citation `yousefi2020modulation' on page 1 undefined on
 input line 122.


Package natbib Warning: Citation `verwey2020experimental' on page 1 undefined o
n input line 127.


Package natbib Warning: Citation `lupo2019immersed' on page 1 undefined on inpu
t line 127.


Package natbib Warning: Citation `lupo2020direct' on page 1 undefined on input 
line 127.


Underfull \vbox (badness 1137) has occurred while \output is active
Underfull \hbox (badness 10000) has occurred while \output is active

[1{/usr/local/texlive/2019/texmf-var/fonts/map/pdftex/updmap/pdftex.map}
Non-PDF special ignored!
<special> papersize=174mm,247mm
]
Underfull \vbox (badness 10000) has occurred while \output is active [2]

Package natbib Warning: Citation `scapin2020volume' on page 3 undefined on inpu
t line 139.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 3 undefined on
 input line 140.


Package natbib Warning: Citation `maxey1982distortion' on page 3 undefined on i
nput line 140.


Package natbib Warning: Citation `wang2019vaporization' on page 3 undefined on 
input line 140.


Package natbib Warning: Citation `ni2021numerical' on page 3 undefined on input
 line 140.


Underfull \vbox (badness 10000) has occurred while \output is active [3]

Package natbib Warning: Citation `majda1985derivation' on page 4 undefined on i
nput line 159.


Package natbib Warning: Citation `reid1987properties' on page 4 undefined on in
put line 174.

[4]pdfTeX warning (ext4): destination with the same identifier (name{equation.2
.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                  [5]

Package natbib Warning: Citation `leonard1979stable' on page 6 undefined on inp
ut line 254.


Package natbib Warning: Citation `scapin2020volume' on page 6 undefined on inpu
t line 254.


Package natbib Warning: Citation `dalla2020interface' on page 6 undefined on in
put line 254.


Package natbib Warning: Citation `costa2018fft' on page 6 undefined on input li
ne 255.

[6 <./figures/fig1-eps-converted-to.pdf>]

Package natbib Warning: Citation `ii2012interface' on page 7 undefined on input
 line 258.


Package natbib Warning: Citation `rosti2019numerical' on page 7 undefined on in
put line 258.


Package natbib Warning: Citation `scapin2020volume' on page 7 undefined on inpu
t line 263.


Package natbib Warning: Citation `ii2012interface' on page 7 undefined on input
 line 270.

[7]

Package natbib Warning: Citation `scapin2020volume' on page 8 undefined on inpu
t line 282.


Package natbib Warning: Citation `scapin2020volume' on page 8 undefined on inpu
t line 291.


Package natbib Warning: Citation `scapin2020volume' on page 8 undefined on inpu
t line 295.

[8]

Package natbib Warning: Citation `gerz1989direct' on page 9 undefined on input 
line 314.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 9 undefined on
 input line 314.


Package natbib Warning: Citation `tanaka2017effect' on page 9 undefined on inpu
t line 319.


Package natbib Warning: Citation `scapin2020volume' on page 9 undefined on inpu
t line 330.


Package natbib Warning: Citation `gerz1989direct' on page 9 undefined on input 
line 330.

[9]

Package natbib Warning: Citation `dalla2020interface' on page 10 undefined on i
nput line 355.


Package natbib Warning: Citation `demou2019low' on page 10 undefined on input l
ine 356.


Package natbib Warning: Citation `dalla2020interface' on page 10 undefined on i
nput line 356.

[10]

Package natbib Warning: Citation `rosti2019droplets' on page 11 undefined on in
put line 383.


Package natbib Warning: Citation `dodd2014fast' on page 11 undefined on input l
ine 384.


Package natbib Warning: Citation `motheau2016high' on page 11 undefined on inpu
t line 385.


Package natbib Warning: Citation `dalla2020interface' on page 11 undefined on i
nput line 385.


Package natbib Warning: Citation `tanaka2017effect' on page 11 undefined on inp
ut line 385.


Package natbib Warning: Citation `rosti2019droplets' on page 11 undefined on in
put line 385.


Package natbib Warning: Citation `scapin2020volume' on page 11 undefined on inp
ut line 398.


Package natbib Warning: Citation `dalla2020interface' on page 11 undefined on i
nput line 398.

[11]
Overfull \hbox (9.16872pt too wide) in paragraph at lines 425--479
[]$[]$  $[]$ 

Package natbib Warning: Citation `hubbard1975droplet' on page 12 undefined on i
nput line 482.

[12]

Package natbib Warning: Citation `sekimoto2016direct' on page 13 undefined on i
nput line 484.


Package natbib Warning: Citation `scapin2020volume' on page 13 undefined on inp
ut line 484.


Package natbib Warning: Citation `abramzon1989droplet' on page 13 undefined on 
input line 491.


Package natbib Warning: Citation `lupo2019immersed' on page 13 undefined on inp
ut line 491.


Package natbib Warning: Citation `lupo2020direct' on page 13 undefined on input
 line 491.


Package natbib Warning: Citation `hubbard1975droplet' on page 13 undefined on i
nput line 491.


Package natbib Warning: Citation `langmuir1918evaporation' on page 13 undefined
 on input line 491.


Package natbib Warning: Citation `piedra2015numerical' on page 13 undefined on 
input line 491.

[13] [14 <./figures/fig2-eps-converted-to.pdf> <./figures/fig3-eps-converted-to
.pdf>]

Package natbib Warning: Citation `birouk2006current' on page 15 undefined on in
put line 549.


Package natbib Warning: Citation `abramzon1989droplet' on page 15 undefined on 
input line 549.


Package natbib Warning: Citation `ranz1952evaporation' on page 15 undefined on 
input line 555.


Package natbib Warning: Citation `birouk2006current' on page 15 undefined on in
put line 555.

[15 <./figures/fig4-eps-converted-to.pdf> <./figures/fig5-eps-converted-to.pdf>
 <./figures/fig6-eps-converted-to.pdf>]

Package natbib Warning: Citation `ranz1952evaporation' on page 16 undefined on 
input line 563.


Package natbib Warning: Citation `wang2021direct' on page 16 undefined on input
 line 563.


Package natbib Warning: Citation `ng2021growth' on page 16 undefined on input l
ine 563.


Package natbib Warning: Citation `ng2021growth' on page 16 undefined on input l
ine 563.


Package natbib Warning: Citation `gokalp1992mass' on page 16 undefined on input
 line 564.


Package natbib Warning: Citation `abramzon1989droplet' on page 16 undefined on 
input line 574.


Package natbib Warning: Citation `birouk2006current' on page 16 undefined on in
put line 574.


Package natbib Warning: Citation `abramzon1989droplet' on page 16 undefined on 
input line 580.


Package natbib Warning: Citation `lupo2020uncertainty' on page 16 undefined on 
input line 582.

[16 <./figures/fig7-eps-converted-to.pdf> <./figures/fig8-eps-converted-to.pdf>
] [17 <./figures/fig9-eps-converted-to.pdf> <./figures/fig10-eps-converted-to.p
df>]

Package natbib Warning: Citation `mees2020statistical' on page 18 undefined on 
input line 610.


Package natbib Warning: Citation `lupo2020direct' on page 18 undefined on input
 line 610.


Package natbib Warning: Citation `verwey2018fuel' on page 18 undefined on input
 line 616.


Package natbib Warning: Citation `verwey2020experimental' on page 18 undefined 
on input line 616.


Package natbib Warning: Citation `marti2017evaporation' on page 18 undefined on
 input line 616.


Package natbib Warning: Citation `birouk2006current' on page 18 undefined on in
put line 616.

[18]

Package natbib Warning: Citation `ni2021numerical' on page 19 undefined on inpu
t line 707.

[19 <./figures/fig11-eps-converted-to.pdf> <./figures/fig12-eps-converted-to.pd
f>]

Package natbib Warning: Citation `wong1992internal' on page 20 undefined on inp
ut line 749.


Package natbib Warning: Citation `pinheiro2019ethanol' on page 20 undefined on 
input line 749.


Underfull \vbox (badness 2781) has occurred while \output is active [20 <./figu
res/fig13-eps-converted-to.pdf> <./figures/fig14-eps-converted-to.pdf> <./figur
es/fig15-eps-converted-to.pdf>] [21 <./figures/fig16-eps-converted-to.pdf> <./f
igures/fig17-eps-converted-to.pdf> <./figures/fig18-eps-converted-to.pdf> <./fi
gures/fig19-eps-converted-to.pdf>] [22 <./figures/fig20-eps-converted-to.pdf> <
./figures/fig21-eps-converted-to.pdf>]

Package natbib Warning: Citation `tonini2013exact' on page 23 undefined on inpu
t line 831.


Package natbib Warning: Citation `saenz2017dynamics' on page 23 undefined on in
put line 831.

[23 <./figures/fig22-eps-converted-to.pdf> <./figures/fig23-eps-converted-to.pd
f> <./figures/fig24-eps-converted-to.pdf>] [24 <./figures/fig25-eps-converted-t
o.pdf> <./figures/fig26-eps-converted-to.pdf> <./figures/fig27-eps-converted-to
.pdf>] [25 <./figures/fig28-eps-converted-to.pdf> <./figures/fig29-eps-converte
d-to.pdf>]

Package natbib Warning: Citation `kasbaoui2017algorithm' on page 26 undefined o
n input line 880.


Package natbib Warning: Citation `ranz1952evaporation' on page 26 undefined on 
input line 890.


Package natbib Warning: Citation `mees2020statistical' on page 26 undefined on 
input line 890.


Package natbib Warning: Citation `tonini2013exact' on page 26 undefined on inpu
t line 900.


Package natbib Warning: Citation `saenz2017dynamics' on page 26 undefined on in
put line 900.

[26 <./figures/fig30-eps-converted-to.pdf>]
Overfull \hbox (16.66757pt too wide) in paragraph at lines 916--922
[]\OT1/cmr/m/n/10 N. Scapin, https://orcid.org/0000-0002-1330-3348; F. Dalla Ba
rba, https://orcid.org/0000-

Underfull \hbox (badness 1960) in paragraph at lines 916--922
\OT1/cmr/m/n/10 0002-4262-0537; Gi-an-domenico Lupo, https://orcid.org/0000-000
2-1095-118X; M.E.
[27]

Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 944.


Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 952.


Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 960.


Package natbib Warning: Citation `reid1987properties' on page 28 undefined on i
nput line 968.

[28]

Package natbib Warning: Citation `span1996new' on page 29 undefined on input li
ne 980.


Package natbib Warning: Citation `span1996new' on page 29 undefined on input li
ne 985.


Package natbib Warning: Citation `reid1987properties' on page 29 undefined on i
nput line 988.


Package natbib Warning: Citation `majda1985derivation' on page 29 undefined on 
input line 992.


Package natbib Warning: Citation `dodd2021analysis' on page 29 undefined on inp
ut line 992.

[29]

Package natbib Warning: Citation `dodd2021analysis' on page 30 undefined on inp
ut line 1031.


Package natbib Warning: Citation `motheau2016high' on page 30 undefined on inpu
t line 1038.


Package natbib Warning: Citation `reid1987properties' on page 30 undefined on i
nput line 1038.

[30]

Package natbib Warning: Citation `lupo2019immersed' on page 31 undefined on inp
ut line 1056.

[31]

Package natbib Warning: Citation `scapin2020volume' on page 32 undefined on inp
ut line 1101.


Package natbib Warning: Citation `ni2021numerical' on page 32 undefined on inpu
t line 1148.


Package natbib Warning: Citation `ni2021numerical' on page 32 undefined on inpu
t line 1148.

[32]

Package natbib Warning: Citation `verwey2018fuel' on page 33 undefined on input
 line 1148.


Package natbib Warning: Citation `dodd2021analysis' on page 33 undefined on inp
ut line 1148.


Package natbib Warning: Citation `podvigina1994non' on page 33 undefined on inp
ut line 1148.


Package natbib Warning: Citation `verwey2018fuel' on page 33 undefined on input
 line 1148.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 33 undefined o
n input line 1151.


Package natbib Warning: Citation `gerz1989direct' on page 33 undefined on input
 line 1151.


Package natbib Warning: Citation `maxey1982distortion' on page 33 undefined on 
input line 1151.


Package natbib Warning: Citation `isaza2009asymptotic' on page 33 undefined on 
input line 1151.

[33 <./figures/fig31-eps-converted-to.pdf> <./figures/fig32-eps-converted-to.pd
f>]

Package natbib Warning: Citation `kasbaoui2017algorithm' on page 34 undefined o
n input line 1155.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 34 undefined o
n input line 1161.


Package natbib Warning: Citation `maxey1982distortion' on page 34 undefined on 
input line 1161.


Package natbib Warning: Citation `gerz1989direct' on page 34 undefined on input
 line 1182.


Underfull \hbox (badness 1642) in paragraph at lines 1180--1183
\OT1/cmr/m/n/10 Following the ap-proach pro-posed by \OT1/cmr/bx/n/10 ?\OT1/cmr
/m/n/10 , we set $[]([]\OML/cmm/m/it/10 ; \OT1/cmr/bx/n/10 k[]\OT1/cmr/m/n/10 )
 = [] [](\OML/cmm/m/it/10 i\OT1/cmr/bx/n/10 k[] \OMS/cmsy/m/n/10 ^^A \OT1/cmr/b
x/n/10 x\OT1/cmr/m/n/10 )$

Underfull \hbox (badness 2653) in paragraph at lines 1180--1183
\OT1/cmr/m/n/10 and $[]([]\OML/cmm/m/it/10 ; \OT1/cmr/bx/n/10 k[]\OT1/cmr/m/n/1
0 ) = [] [](\OML/cmm/m/it/10 i\OT1/cmr/bx/n/10 k[] \OMS/cmsy/m/n/10 ^^A \OT1/cm
r/bx/n/10 x\OT1/cmr/m/n/10 )$. More-over, by us-ing the iden-tity
[34pdfTeX warning (ext4): destination with the same identifier (name{equation.D
.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1186 \end{equation}
                     pdfTeX warning (ext4): destination with the same identifie
r (name{equation.D.2}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1186 \end{equation}
                      <./figures/fig33-eps-converted-to.pdf> <./figures/fig34-e
ps-converted-to.pdf>]

Package natbib Warning: Citation `gerz1989direct' on page 35 undefined on input
 line 1199.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 35 undefined o
n input line 1230.


Package natbib Warning: Citation `tanaka2017effect' on page 35 undefined on inp
ut line 1231.


Package natbib Warning: Citation `yousefi2020modulation' on page 35 undefined o
n input line 1231.


Package natbib Warning: Citation `kasbaoui2017algorithm' on page 35 undefined o
n input line 1231.

[35] (./jfm.bbl [36 <./figures/fig35-eps-converted-to.pdf> <./figures/fig36-eps
-converted-to.pdf>] [37 <./figures/fig37-eps-converted-to.pdf> <./figures/fig38
-eps-converted-to.pdf> <./figures/fig39-eps-converted-to.pdf>]
Underfull \hbox (badness 3333) in paragraph at lines 21--25
[]\OT1/cmr/m/sc/9 Balachandar, S, Za-leski, Stephane, Sol-dati, Al-fredo, Ah-ma
di, Goodarz &

Underfull \hbox (badness 1412) in paragraph at lines 73--79
[]\OT1/cmr/m/sc/9 Dauxois, Thierry, Pea-cock, Thomas, Bauer, Pe-ter, Caulfield,
 Colm-cille P,

Underfull \hbox (badness 2326) in paragraph at lines 73--79
\OT1/cmr/m/sc/9 Paul F, Meiburg, Eckart & oth-ers \OT1/cmr/m/n/9 2021 Con-front
ing grand chal-lenges in
[38]
Underfull \vbox (badness 3690) has occurred while \output is active [39]
Underfull \hbox (badness 1874) in paragraph at lines 289--293
[]\OT1/cmr/m/sc/9 Reveillon, Julien & De-moulin, Fran[]ois-Xavier \OT1/cmr/m/n/
9 2007 Ef-fects of the pref-er-en-tial

Underfull \vbox (badness 10000) has occurred while \output is active [40])

Package natbib Warning: There were undefined citations.

[41] (./jfm.aux

Package natbib Warning: Citation(s) may have changed.
(natbib)                Rerun to get citations correct.

)

LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information){/usr/local/texlive/2019/te
xmf-dist/fonts/enc/dvips/cm-super/cm-super-ts1.enc}</usr/local/texlive/2019/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2019/texm
f-dist/fonts/type1/public/amsfonts/cm/cmbx12.pfb></usr/local/texlive/2019/texmf
-dist/fonts/type1/public/amsfonts/cm/cmbx7.pfb></usr/local/texlive/2019/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmbx8.pfb></usr/local/texlive/2019/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmbx9.pfb></usr/local/texlive/2019/texmf-dist/
fonts/type1/public/amsfonts/cm/cmcsc10.pfb></usr/local/texlive/2019/texmf-dist/
fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2019/texmf-dist/f
onts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2019/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2019/texmf-dist/font
s/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2019/texmf-dist/fonts/
type1/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2019/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type
1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/
public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmr6.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public
/amsfonts/cm/cmr7.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/am
sfonts/cm/cmr9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfon
ts/cm/cmsy5.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts
/cm/cmsy6.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/c
m/cmsy7.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/
cmsy9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/cm
ti10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/cmt
i8.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/cmti9
.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/symbols/ms
am10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/cm-super/sfrm10
00.pfb>
Output written on jfm.pdf (41 pages, 8954919 bytes).
Transcript written on jfm.log.
pdflatex: unrecognized option '-pdf'
pdflatex: option '-f' is ambiguous; possibilities: '-fmt' '-file-line-error-style' '-file-line-error'
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./jfm.tex
LaTeX2e <2019-10-01> patch level 3
(./jfm.cls
Document Class: jfm 2007/03/13 v1.28 Journal of Fluid Mechanics document class
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/etoolbox/etoolbox.sty)

Found the 'amsbsy' package on the system, using it.

(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsbsy.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsgen.sty))

Found AMS Euler Roman fonts on the system, but you dont seem to have the
'upmath' package installed. JFM.cls can take advantage of these fonts,
if you use 'upmath' package.



Found AMS Symbol fonts on the system, using the 'amssymb' package.

(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/amsfonts.sty)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/lineno/lineno.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2019/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hycolor/hycolor.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/hycolor/xcolor-patch.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/oberdiek/hopatch.sty)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2019/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2019/texmf-dist/tex/generic/atbegshi/atbegshi.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2019/texmf-dist/tex/latex/atveryend/atveryend.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2019/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2019/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amstext.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/textcomp.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1enc.def
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1enc.dfu)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/nomencl/nomencl.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2019/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2019/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))
(/usr/local/texlive/2019/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/tocbasic.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/scrbase.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/koma-script/scrlfile.sty))))
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2019/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/dvipsnam.def))
(/usr/local/texlive/2019/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/tabularx.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/tools/array.sty

LaTeX Warning: Command \@xhline  has changed.
               Check if current package is valid.

)) (/usr/local/texlive/2019/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/adjustbox.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/adjcalc.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/trimclip.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/collectbox/collectbox.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/adjustbox/tc-pdftex.def))
(/usr/local/texlive/2019/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/varwidth/varwidth.sty))
(/usr/local/texlive/2019/texmf-dist/tex/latex/realboxes/realboxes.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/appendix/appendix.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/cancel/cancel.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/epstopdf-pkg/epstopdf.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/grfext/grfext.sty)
(/usr/local/texlive/2019/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg)))
(./jfm.aux

LaTeX Warning: Label `eqn:veldiv' multiply defined.

) (/usr/local/texlive/2019/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/local/texlive/2019/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
)

Package hyperref Warning: Height of page (\paperheight) is invalid (0.0pt),
(hyperref)                using 11in.

(/usr/local/texlive/2019/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2019/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2019/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./jfm.out) (./jfm.out)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2019/texmf-dist/tex/latex/amsfonts/umsb.fd)
Underfull \vbox (badness 1137) has occurred while \output is active
Underfull \hbox (badness 10000) has occurred while \output is active

[1{/usr/local/texlive/2019/texmf-var/fonts/map/pdftex/updmap/pdftex.map}
Non-PDF special ignored!
<special> papersize=174mm,247mm
]
Underfull \vbox (badness 10000) has occurred while \output is active [2]
Underfull \vbox (badness 10000) has occurred while \output is active [3]
[4]pdfTeX warning (ext4): destination with the same identifier (name{equation.2
.1}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.2}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                 pdfTeX warning (ext4): destination with the same identifier (n
ame{equation.2.3}) has been already used, duplicate ignored
<to be read again> 
                   \relax 
l.190 \end{align}
                  [5]
Underfull \vbox (badness 4927) has occurred while \output is active [6 <./figur
es/fig1-eps-converted-to.pdf>] [7] [8] [9]
Underfull \vbox (badness 7151) has occurred while \output is active [10]
[11]
Overfull \hbox (9.16872pt too wide) in paragraph at lines 425--479
[]$[]$  $[]$ 
[12]
Underfull \vbox (badness 7012) has occurred while \output is active [13]
Underfull \vbox (badness 10000) has occurred while \output is active [14]
[15 <./figures/fig2-eps-converted-to.pdf> <./figures/fig3-eps-converted-to.pdf>
 <./figures/fig4-eps-converted-to.pdf>] [16 <./figures/fig5-eps-converted-to.pd
f> <./figures/fig6-eps-converted-to.pdf> <./figures/fig7-eps-converted-to.pdf> 
<./figures/fig8-eps-converted-to.pdf>] [17] [18 <./figures/fig9-eps-converted-t
o.pdf> <./figures/fig10-eps-converted-to.pdf>] [19 <./figures/fig11-eps-convert
ed-to.pdf> <./figures/fig12-eps-converted-to.pdf>] [20 <./figures/fig13-eps-con
verted-to.pdf> <./figures/fig14-eps-converted-to.pdf> <./figures/fig15-eps-conv
erted-to.pdf>] [21 <./figures/fig16-eps-converted-to.pdf> <./figures/fig17-eps-
converted-to.pdf> <./figures/fig18-eps-converted-to.pdf> <./figures/fig19-eps-c
onverted-to.pdf>] [22 <./figures/fig20-eps-converted-to.pdf> <./figures/fig21-e
ps-converted-to.pdf>] [23 <./figures/fig22-eps-converted-to.pdf> <./figures/fig
23-eps-converted-to.pdf> <./figures/fig24-eps-converted-to.pdf>] [24 <./figures
/fig25-eps-converted-to.pdf> <./figures/fig26-eps-converted-to.pdf>] [25 <./fig
ures/fig27-eps-converted-to.pdf> <./figures/fig28-eps-converted-to.pdf>]
[26 <./figures/fig29-eps-converted-to.pdf> <./figures/fig30-eps-converted-to.pd
f>] [27]
Overfull \hbox (16.66757pt too wide) in paragraph at lines 916--922
[]\OT1/cmr/m/n/10 N. Scapin, https://orcid.org/0000-0002-1330-3348; F. Dalla Ba
rba, https://orcid.org/0000-

Underfull \hbox (badness 1960) in paragraph at lines 916--922
\OT1/cmr/m/n/10 0002-4262-0537; Gi-an-domenico Lupo, https://orcid.org/0000-000
2-1095-118X; M.E.
[28] [29] [30] [31] [32] [33 <./figures/fig31-eps-converted-to.pdf> <./figures/
fig32-eps-converted-to.pdf>] [34 <./figures/fig33-eps-converted-to.pdf> <./figu
res/fig34-eps-converted-to.pdf>] [35pdfTeX warning (ext4): destination with the
 same identifier (name{equation.D.1}) has been already used, duplicate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1198 ...and  old time level, $n$ and $n-1$. \par
                                                  pdfTeX warning (ext4): destin
ation with the same identifier (name{equation.D.2}) has been already used, dupl
icate ignored

\AtBegShi@Output ...ipout \box \AtBeginShipoutBox 
                                                  \fi \fi 
l.1198 ...and  old time level, $n$ and $n-1$. \par
                                                  ] [36] (./jfm.bbl [37 <./figu
res/fig35-eps-converted-to.pdf> <./figures/fig36-eps-converted-to.pdf> <./figur
es/fig37-eps-converted-to.pdf>]
Underfull \hbox (badness 3333) in paragraph at lines 21--25
[]\OT1/cmr/m/sc/9 Balachandar, S, Za-leski, Stephane, Sol-dati, Al-fredo, Ah-ma
di, Goodarz &
[38 <./figures/fig38-eps-converted-to.pdf> <./figures/fig39-eps-converted-to.pd
f>]
Underfull \hbox (badness 1412) in paragraph at lines 73--79
[]\OT1/cmr/m/sc/9 Dauxois, Thierry, Pea-cock, Thomas, Bauer, Pe-ter, Caulfield,
 Colm-cille P,

Underfull \hbox (badness 2326) in paragraph at lines 73--79
\OT1/cmr/m/sc/9 Paul F, Meiburg, Eckart & oth-ers \OT1/cmr/m/n/9 2021 Con-front
ing grand chal-lenges in

Underfull \vbox (badness 6380) has occurred while \output is active [39]
Underfull \hbox (badness 1874) in paragraph at lines 289--293
[]\OT1/cmr/m/sc/9 Reveillon, Julien & De-moulin, Fran[]ois-Xavier \OT1/cmr/m/n/
9 2007 Ef-fects of the pref-er-en-tial

Underfull \vbox (badness 10000) has occurred while \output is active [40])
[41] (./jfm.aux)

LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information){/usr/local/texlive/2019/te
xmf-dist/fonts/enc/dvips/cm-super/cm-super-ts1.enc}</usr/local/texlive/2019/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2019/texm
f-dist/fonts/type1/public/amsfonts/cm/cmbx12.pfb></usr/local/texlive/2019/texmf
-dist/fonts/type1/public/amsfonts/cm/cmbx7.pfb></usr/local/texlive/2019/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmbx8.pfb></usr/local/texlive/2019/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmbx9.pfb></usr/local/texlive/2019/texmf-dist/
fonts/type1/public/amsfonts/cm/cmcsc10.pfb></usr/local/texlive/2019/texmf-dist/
fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2019/texmf-dist/f
onts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2019/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2019/texmf-dist/font
s/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2019/texmf-dist/fonts/
type1/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2019/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type
1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/
public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmr6.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public
/amsfonts/cm/cmr7.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/am
sfonts/cm/cmr9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfon
ts/cm/cmsy5.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts
/cm/cmsy6.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/c
m/cmsy7.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/
cmsy9.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/cm
ti10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/cmt
i8.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/cm/cmti9
.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/amsfonts/symbols/ms
am10.pfb></usr/local/texlive/2019/texmf-dist/fonts/type1/public/cm-super/sfrm10
00.pfb>
Output written on jfm.pdf (41 pages, 8969464 bytes).
Transcript written on jfm.log.

